On Bayesian data assimilation for PDEs with ill-posed forward problems

We study Bayesian data assimilation (filtering) for time-evolution PDEs, for which the underlying forward problem may be very unstable or ill-posed. Such PDEs, which include the Navier-Stokes equations of fluid dynamics, are characterized by a high sensitivity of solutions to perturbations of the initial data, a lack of rigorous global well-posedness results as well as possible non-convergence of numerical approximations. Under very mild and readily verifiable general hypotheses on the forward solution operator of such PDEs, we prove that the posterior measure expressing the solution of the Bayesian filtering problem is stable with respect to perturbations of the noisy measurements, and we provide quantitative estimates on the convergence of approximate Bayesian filtering distributions computed from numerical approximations. For the Navier-Stokes equations, our results imply uniform stability of the filtering problem even at arbitrarily small viscosity, when the underlying forward problem may become ill-posed, as well as the compactness of numerical approximants in a suitable metric on time-parametrized probability measures.

==> diagram.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,386); %set diagram left start at 0, and has height of 386

%Straight Lines [id:da9902773307713919] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (464,289) -- (465.2,358.93) ;
\draw [shift={(465.23,360.93)}, rotate = 269.02] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(464,289)}, rotate = 269.02] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
%Straight Lines [id:da9029514258431245] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (464.23,273.93) -- (178.13,369.3) ;
\draw [shift={(176.23,369.93)}, rotate = 341.57] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw    (148,58) -- (176,58) -- (176,87) -- (148,87) -- cycle  ;
\draw (151,62.4) node [anchor=north west][inner sep=0.75pt]    {$\mu ^{\Delta }_{0}$};
% Text Node
\draw    (446,58) -- (482,58) -- (482,87) -- (446,87) -- cycle  ;
\draw (449,62.4) node [anchor=north west][inner sep=0.75pt]    {$\mu ^{\Delta ,y_1 }_{0}$};

% Text Node
\draw    (148,158) -- (176,158) -- (176,187) -- (148,187) -- cycle  ;
\draw (151,162.4) node [anchor=north west][inner sep=0.75pt]    {$\mu ^{\Delta }_{1}$};
% Text Node
\draw    (446,158) -- (482,158) -- (482,187) -- (446,187) -- cycle  ;
\draw (449,162.4) node [anchor=north west][inner sep=0.75pt]    {$\mu ^{\Delta ,y_2 }_{1}$};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (148,258) -- (176,258) -- (176,287) -- (148,287) -- cycle  ;
\draw (151,262.4) node [anchor=north west][inner sep=0.75pt]    {$\mu ^{\Delta }_{2}$};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (448,258) -- (484,258) -- (484,287) -- (448,287) -- cycle  ;
\draw (451,262.4) node [anchor=north west][inner sep=0.75pt]    {$\mu ^{\Delta ,y_3 }_{2}$};
% Connection
\draw    (176,72.5) -- (444,72.5) ;
\draw [shift={(446,72.5)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Connection
\draw    (446,78.46) -- (177.9,167.24) ;
\draw [shift={(176,167.86)}, rotate = 341.68] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Connection
\draw    (176,172.5) -- (444,172.5) ;
\draw [shift={(446,172.5)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Connection
\draw    (446,178.46) -- (177.9,267.24) ;
\draw [shift={(176,267.86)}, rotate = 341.68] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Connection
\draw    (464,89) -- (464,156) ;
\draw [shift={(464,158)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(464,89)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
% Connection
\draw    (464.33,189) -- (465.67,256) ;
\draw [shift={(465.71,258)}, rotate = 268.85] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(464.33,189)}, rotate = 268.85] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
% Connection
\draw    (176,272.5) -- (446,272.5) ;
\draw [shift={(448,272.5)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (312, 71) circle [x radius= 87.68, y radius= 15.56]   ;
\draw (251,62.4) node [anchor=north west][inner sep=0.75pt]    {$y_{1} \ =\ \mathcal{L}_{1}( u) +\eta _{1}$};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (309.5, 126.5) circle [x radius= 28.99, y radius= 19.09]   ;
\draw (290,115.4) node [anchor=north west][inner sep=0.75pt]    {$S^{\Delta }_{\Delta t_{1} ,\#}$};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (312, 170) circle [x radius= 87.68, y radius= 15.56]   ;
\draw (251,161.4) node [anchor=north west][inner sep=0.75pt]    {$y_{2} \ =\ \mathcal{L}_{2}( u) +\eta _{2}$};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (309.5, 226.5) circle [x radius= 28.99, y radius= 19.09]   ;
\draw (290,215.4) node [anchor=north west][inner sep=0.75pt]    {$S^{\Delta }_{\Delta t_{2} ,\#}$};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (310.5, 326.5) circle [x radius= 28.99, y radius= 19.09]   ;
\draw (291,315.4) node [anchor=north west][inner sep=0.75pt]    {$S^{\Delta }_{\Delta t_{3} ,\#}$};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (312, 269) circle [x radius= 87.68, y radius= 15.56]   ;
\draw (251,260.4) node [anchor=north west][inner sep=0.75pt]    {$y_{3} \ =\ \mathcal{L}_{3}( u) +\eta _{3}$};
\end{tikzpicture}


==> filtering_diagram.tex <==


\begin{tikzcd}
\ldots \arrow[r]
&
\nu^{\Delta,Y_{j-1}}_{t_{j-1}} \arrow[r] \arrow[d,"y_{j}",orange]
&
\nu^{\Delta,Y_{j}}_{t_{j}} \arrow[r] \arrow[d,"y_{j+1}",orange]
&
\nu^{\Delta,Y_{j+1}}_{t_{j+1}} \arrow[r]
& 
\ldots 
\\
&
\nu^{\Delta,Y_{j}}_{t_{j-1}} \arrow[ur,blue]
&
\nu^{\Delta,Y_{j+1}}_{t_{j}} \arrow[ur,blue]
&
& 
\end{tikzcd}


%% Text Node
%\draw (190,60.4) node [anchor=north west][inner sep=0.75pt]    {$\nu ^{\Delta ,Y_{j-1}}_{t_{j-1}}$};
%% Text Node
%\draw (190,146.4) node [anchor=north west][inner sep=0.75pt]    {$\nu ^{\Delta ,Y_{j}}_{t_{j-1}}$};
%% Text Node
%\draw (300,60.4) node [anchor=north west][inner sep=0.75pt]    {$\nu ^{\Delta ,Y_{j}}_{t_{j}}$};
%% Text Node
%\draw (300,146.4) node [anchor=north west][inner sep=0.75pt]    {$\nu ^{\Delta ,Y_{j+1}}_{t_{j}}$};
%% Text Node
%\draw (410,60.4) node [anchor=north west][inner sep=0.75pt]    {$\nu ^{\Delta ,Y_{j+1}}_{t_{j+1}}$};
%% Text Node
%\draw (80,60.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,opacity=1 ]  {$\nu ^{\Delta ,Y_{j-2}}_{t_{j-2}}$};
%% Text Node
%\draw (520,60.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,opacity=1 ]  {$\nu ^{\Delta ,Y_{j+2}}_{t_{j+2}}$};


%% Connection
%\draw [line width=0.75]    (242,76) -- (310,76) ;
%\draw [shift={(312,76)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%% Connection
%\draw    (212.88,96) -- (212.63,140) ;
%\draw [shift={(212.62,142)}, rotate = 270.33] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%% Connection
%\draw    (237,145.01) -- (310.36,94.13) ;
%\draw [shift={(312,92.99)}, rotate = 505.26] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%% Connection
%\draw    (336.5,96) -- (336.5,140) ;
%\draw [shift={(336.5,142)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%% Connection
%\draw    (361.15,142) -- (416.3,97.26) ;
%\draw [shift={(417.85,96)}, rotate = 500.95] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%% Connection
%\draw    (361,76) -- (411,76) ;
%\draw [shift={(413,76)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%% Connection
%\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=0.75]    (140,74.57) -- (182,75.39) ;
%\draw [shift={(184,75.43)}, rotate = 181.12] [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%% Connection
%\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (472,76.56) -- (516,77.4) ;
%\draw [shift={(518,77.44)}, rotate = 181.09] [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%
%\end{tikzpicture}

